CoLight: Learning Network-level Cooperation for Traffic Signal Control

Cooperation among the traffic signals enables vehicles to move through intersections more quickly. Conventional transportation approaches implement cooperation by pre-calculating the offsets between two intersections. Such pre-calculated offsets are not suitable for dynamic traffic environments. To enable cooperation of traffic signals, in this paper, we propose a model, CoLight, which uses graph attentional networks to facilitate communication. Specifically, for a target intersection in a network, CoLight can not only incorporate the temporal and spatial influences of neighboring intersections to the target intersection, but also build up index-free modeling of neighboring intersections. To the best of our knowledge, we are the first to use graph attentional networks in the setting of reinforcement learning for traffic signal control and to conduct experiments on the large-scale road network with hundreds of traffic signals. In experiments, we demonstrate that by learning the communication, the proposed model can achieve superior performance against the state-of-the-art methods.

==> README <==
This package provides a class for typesetting publications of the
Association for Computing Machinery.

Your TeX distribution probably includes the latest released version of
this package.  If you decide to install it yourself, please see the
Installation section of the User's Guide.

Please note that the version on Github is a development (or
experimental) version: please download it for testing new features.
The production version is the one on CTAN and ACM sites.


Changes

version 1.08    SIGPLAN reformatting (Matthew Fluet); bug fixes

version 1.09    SIGPLAN: revert caption rules (Matthew Fluet)

version 1.10    Bug fixes

version 1.11    Customization of ACM theorem styles and proof
                environment (Matthew Fluet).

version 1.12    Bug fixes and documentation updates.
                Footnotes rearranged.
                Option natbib is now mostly superfluous: the class
                makes a guess based on the format chosen.

version 1.13    Formatting changes: headers, folios etc.
                Bibliography changes.

version 1.14    Warn about undefined citation styles; move definitions
                of acmauthoryear and acmnumeric citation styles before
                use.

version 1.15    New structured affiliation command.
                New commands for acknowledgements.

version 1.16    Formatting changes for headers and footers.

version 1.17    Formatting changes for margins and lists.  Bug fixes.

version 1.18    Natbib is now the default for all versions.  A unified bib
                file is used for all styles.  Better treatment
                of multiple affiliations.

version 1.19    Include 'Abstract', 'Acknowledgements', and 'References'
                in PDF bookmarks.

version 1.20    Bug fixes, documentation updates

version 1.21    Bibliography changes: added arXiv, some cleanup

version 1.22    Bibliography changes for Aptara backend; should be
                invisible for the users.

version 1.23    Added PACM PL journal option.

version 1.24    Added IMWUT journal option.

version 1.25    Updated PACMPL journal option.

version 1.26    Bug fixes

version 1.27    Bug fixes

version 1.28    Bug fixes: natbib=false now behaves correctly.

version 1.29    Documentation changes.  Head height increased from 12pt to 13pt.
                Removed spurious indent at start of abstract.
                Improved kerning in CCS description list.

version 1.30    Bibtex style now recognizes https:// in doi.
                Added \frenchspacing.
                \department now has an optional hierarchy level.
                Switched to T1 encoding
                Updated IMWUT and PACMPL

version 1.31    Changed default year and month to the current ones
                (thanks to Matteo Riondato)
                Table of contents now works
                Marginalia now work in all formats
                New command \additionalaffiliation
                Documentation changes

version 1.32    New DOI formatting.
                Format siggraph is now obsolete, and sigconf
                is used instead.
                New proceedings title: POMACS.

version 1.33    New option `timestamp' (Michael D. Adams)
                New option `authordraft'
                Documentation updates
                Bug fixes
                We now use Type 1 versions of Libertine fonts even with XeTeX.
                New hook acmart-preload-hook.tex (wizards only!)
                Added new options `obeypunctuation' for \affiliation command
                Added SubmissionID
                Added right line count ruler for two-column formats
                Added workaround for Adobe Acrobat bugs in selection
                Added eid field to the bibliography

version 1.34    Deleted DOI from doi numbers
                Changed bibstrip formatting
                The command \terms is now obsolete
                The rulers in review mode now have continuous numbering

version 1.35    Author-year bib style now uses square brackets.
                Changed defaults for TOG sample
                Price is suppressed for usgov and rightsretained modes.
                Bugs fixed

Version 1.36    Bug fixes
                Moved PACMPL to acmlarge format
                New journal: PACMHCI
                Added the possibility to adjust number of author
                boxes per row in conference formats

Version 1.37    Reduce list indentation (Matthew Fluet)

Version 1.38    Increase default font size for SIGPLAN

Version 1.39    Added \authornotemark commmand

Version 1.40    Bibliography changes
                Added processing of one-compoment ccsdesc nodes
                Bug fixes.
                Made the height a multiple of \baselineskip + \topskip
                Added cleveref
                We no longer print street address in SIGs

Version 1.41    Rearranged bib files
                Added new badges

Version 1.42    Deleted ACM badges
                Bug fixes

Version 1.43    Bug fixes

Version 1.44    Bug fixes.
                Empty DOI and ISBN suppress printing DOI or ISBN lines
                Separated theorem code into acmthm.sty, loaded by default.
                Article number can be set for proceedings.
                New commands: \acmBooktile, \editor.
                Reference citation format updated.

Version 1.45    Workaround for a Libertine bug.  Thanks to LianTze Lim
                from Overleaf

Version 1.46    Bug fixes for bibliography: label width is now calculated
                correctly.
                All PACM now use screen option.  This requires etoolbox.
                Added subtitle to ACM reference format.
                Now acmart is compatible with fontspec.
                \thanks is now obsolete.  The addresses are automatically
                added to the journal version; this can be overriden with
                \authorsaddresses command.
                Deleted the rule at the end of frontmatter for all formats.
                Deleted new line before doi in the reference format.
                Reintegrated theorem code into acmart.dtx (Matthew Fluet)

Version 1.47    New journal: THRI

Version 1.48    Bug fixes
                Review mode now switches on folios
                Code prettying (Michael D. Adams)
                Bibliography changes: @MISC entries no longer have a
                separate date
                Sigch-a sample bibliography renamed
                Bib code cleanup (Zack Weinberg)
                Acmart and version info are added to pdfcreator tag
                \citeyear no longer produces parenthetical year
                Added initial support for Biblatex (Daniel Thomas)
                Added support for IW3C2 conferences

Version 1.49    New jorunal:  DTRAP

Version 1.50    Changes in iw3c2w3 and iw3c2w3g

Version 1.51    Journal footers now use abbreviated journal titles.
                Corrected the bug with acmPrice.
                Do not show price when copyright is set to iw3c2w3 and iw3c2w3g.
                The package now is compatible with polyglossia (Joachim Breitner).
                Slightly reworded copyright statements.

Version 1.52    Another rewording of licenses

Version 1.53    New journals: PACMCGIT, TIOT, TDSCI

Version 1.54    New option: 'noacm' (Gabriel Scherer)
                Deleted indent for subsubsection (suggested by Ross Moore)
                Suppressed some obscurious warning in BibTeX processing
                Suppressed hyperrerf warnings (Paolo G. Giarrusso)
                New code for sections to help with accessibility patches
                (Ross Moore)
                Submission id, if present, is printed in anon mode
                Bug fixes

Version 1.55    Bug fixes
		Font changes for SIGCHI table captions


Version 1.56    Bug fixes
		Added \flushbottom to two column formats (Philip Quinn)
		The final punctuation for the list of concepts
		is now period instead of semilcolon (Philip Quinn)
		New command \Description to describe images for visually
		impaired users.

Version 1.57    Change of \baselinestretch now produces an error
		Booktabs is now always loaded
		Added option `balance' to balance last page in two-column mode
		E-mail is no longer split in addresses
		New samples (Stephen Spencer)

==> addendum.tex <==
% !TEX root = main.tex
\section{Addendum}
\subsection{Complexity Analysis\label{sec:addendum_complexity}}

\subsection{Preprocessing of Real-world Data\label{addendum:real_data}}

\subsection{Attention Study}

\begin{figure}[t!]
  \centering
  \subfigure[Road network]{\label{fig:arterial_network}
%   \includegraphics[width=0.21\textwidth]{1x3_case_study.pdf}}
  \includegraphics[width=0.21\textwidth]{1_3_network_new.pdf}}
  \subfigure[Intersection 0]{\label{fig:attention_1x3_0} \includegraphics[width=0.21\textwidth]{attention_1x3_0.pdf}}
  \subfigure[Intersection 1]{\label{fig:attention_1x3_1} \includegraphics[width=0.21\textwidth]{attention_1x3_1.pdf}}
  \subfigure[Intersection 2]{\label{fig:attention_1x3_2} \includegraphics[width=0.21\textwidth]{attention_1x3_2.pdf}}
  \caption{Spatial difference of attention distribution learned by \GAT during training process on \arterial.}
  \label{fig:attention_1x3}
\vspace{-3mm}
\end{figure}
\subsubsection{Synthetic Arterial}
As shown in Figure~\ref{fig:attention_1x3}, a synthetic arterial \arterial with three intersections is used and we analyze the attention distribution for all the intersections. The traffic flow (denoted by straight red lines with arrows for direction) along the arterial is uni-directional, making \emph{Inter \#0} as the upstream of \emph{Inter \#1} and \emph{\#2}. We have the following observations:
~\noindent\\$\bullet$
In Figure~\ref{fig:attention_1x3_0}, \emph{Inter \#0} pays most of its attention on traffic condition of itself, which meets with the fact that the downstream \emph{Inter \#2} and \emph{\#3} have little impact on the policy of the upstream \emph{Inter \#0}.
~\noindent\\$\bullet$
Figure~\ref{fig:attention_1x3_1} shows that \emph{Inter \#1} pays a remarkable attention on \emph{Inter \#0} compared with \emph{Inter \#2}. Such attention distribution for cooperation is reasonable as there are no side roads for \emph{Inter \#1} and the major traffic comes from \emph{Inter \#1}'s upstream \emph{Inter \#0}.
~\noindent\\$\bullet$
In Figure~\ref{fig:attention_1x3_2}, the downstream \emph{Inter \#2} cares most about its own traffic flow while automatically allocating appropriate attention to two upstream intersections.



==> overview.tex <==
\section{Overview of \GAT Framework}
% \subsection{Multi-hop Dynamic Coordination}
% \weinan{what do you mean by overview? Overview of the framework?}


Figure~\ref{fig:framework} demonstrates the scenario of applying the proposed \GAT 
% \weinan{The \GAT term is not explained previously.} 
model to intersections at Hell's Kitchen, Manhattan, where the streets and avenues only accommodate one-way traffic. 

In Fig.~\ref{fig:framework}(a), the \GAT agent selects the green phase for intersection 9-49 (9-th Avenue, West 49-th Street) in three steps. Firstly, observations of all the intersections are embedded concurrently, where the complex inherent structure and regularities of their respective surrounding environment are learned and mapped into a high-dimensional latent space. Secondly, cooperation within the neighborhood is implemented layerwise by learning the attention scores ($\alpha$) and summarizing the contributions ($hm$) of the neighboring intersections to the target intersection 9-49. Lastly, the agent predicts q-values according to the cooperation representation and takes actions with the $\epsilon$-greedy strategy by combining exploration ($\epsilon$ probability for a random action) and exploitation ($(1-\epsilon)$ probability for the action with the maximum q-value).

% In MARL environment, individual RL agents append the neighbors' states to its own as input and feed it to the neural network for action prediction~\cite{Wier00}. With shared network parameters, previously proposed \oneModelNeighbor method similarly takes the nearby agents into consideration by concatenating several state vectors at input stage~\cite{ALUK10}. However, such state combination at network input limits the scope of nearby intersections to only adjacent ones. Meanwhile, the purely expansion of input space without any highlight on some specific segment increases the burden of the neural net to learn the optimal policy.

% To help the agent ``see'' a broader neighborhood status, some work leverages the \GCN network to emphasize the adjacent information by multiplying the original activation with an extra variant of the adjacent matrix ($\hat A$) in each hidden layer~\cite{GCN18}. In the network, the activated vector in the $l$-th hidden layer summarizes information of the adjacent intersections' last hidden vectors (in the $(l\text{-}1)$-th layer), which deliver more distant intersections' message (in the $(l\text{-}2)$-th layer) from the view of the original target intersection. The deeper the hidden layers, the broader the view scope of the target intersection. However, the emphasize on nearby intersections is determined by the pre-defined adjacent matrix, which is unadaptable and especially inefficient when the dynamic traffic deserves more attention for making a signal policy than the static geographic information.

The proposed \GAT method is actually a \emph{multi-hop dynamic cooperation} system, which has a broad view of the surrounding environment and takes the message from the nearby intersections with flexible attention according to the traffic at the same time.
% Figure~\ref{fig:framework}(b)(c) shows the \GAT's multi-hop and flexibility in the real-world scenario. 
% As Fig.~\ref{fig:framework}(b)(c) illustrates, In the beginning, the agent for intersection $9\text{-}49$ only knows its own traffic condition.
After the observation embedding of all intersections flow into the first NCvA (Neighborhood Cooperation via Attention) 
% \weinan{NCvA term is not explained.}
layer (shown in Fig.~\ref{fig:framework}(b)), intersection $9\text{-}49$ acquires the knowledge of adjacent intersections (intersection $9\text{-}48$, $9\text{-}50$, $10\text{-}49$ and $8\text{-}49$) directly. Meanwhile, the emphasizes on the four neighbors are quite distinct due to the one-way running traffic (north to south in 9-th Avenue, east to west in West 49-th Street), e.g., a higher attention score for intersection $9\text{-}50$ (upstream, red marked) than for $9\text{-}48$ (downstream, green marked). Since the hidden states of adjacent neighbors from the first NCvA layer carry their respective neighborhood message, then in the second NCvA layer (shown in Fig.~\ref{fig:framework}(c)), the observation area for intersection $9\text{-}49$ has significantly expanded, with traffic condition from 8 intersections one-hop away covered. Such additional information helps the target intersection $9\text{-}49$ learn the flow trend and rely more on the upstream intersections but less on the downstream to take actions. Hence the attention scores on intersection $9\text{-}50$ and $8\text{-}49$ grow higher while those on intersection $10\text{-}49$ and $9\text{-}48$ become lower. Two hidden NCvA layers offer the agent the chance to detect environment dynamics one-hop away. More hops of view are accessible if the neural network has multiple NCvA layers.  

In conclusion, the graph-level attention employed in the NCvA layers allows the agent to adjust their focus according to the dynamic traffic and sense the environment in a larger scale.
